Integrated Properties of AGB Stars in Unresolved Stellar Populations: Simple Stellar Populations and Star Clusters

The evolution of AGB stars is notoriously complex. The confrontation of AGB population models with observed stellar populations is a useful alternative to the detailed study of individual stars in efforts to converge towards a reliable evolution theory. I review here the impact of studies of star clusters on AGB models and AGB population synthesis, deliberately leaving out any more complex stellar populations. Over the last 10 years, despite much effort, the absolute uncertainties in the predictions of the light emitted by intermediate age populations have not been reduced to a satisfactory level. Observational sample definitions, as well as the combination of the natural variance in AGB properties with small number statistics, are largely responsible for this situation. There is hope that the constraints may soon become strong enough, thanks to large unbiased surveys of star clusters, resolved colour-magnitude diagrams, and new analysis methods that can account for the stochastic nature of AGB populations in clusters.

==> Abstract <==
Title: Integrated Properties of AGB Stars in Unresolved Stellar Populations : 
  Simple Stellar Populations and Star Clusters
Authors: A. Lan\c{c}on (Observatoire de Strasbourg)
Comments: 10 pages. To be published in "Why Galaxies Care about 
  AGB stars II", Vienna, Aug.16-20, 2010, ed. F. Kerschbaum, T. Lebzelter,
  R. Wing (invited talk).

The evolution of AGB stars is notoriously complex. The confrontation of
AGB population models with observed stellar populations is a useful
alternative to the detailed study of individual stars in efforts to converge
towards a reliable evolution theory. I review here the impact of
studies of star clusters on AGB models and AGB population synthesis,
deliberately leaving out any more complex stellar populations. Over the
last 10 years, despite much effort, the absolute uncertainties in the
predictions of the light emitted by intermediate age populations have
not been reduced to a satisfactory level. Observational sample definitions,
as well as the combination of the natural variance in AGB properties with
small number statistics, are largely responsible for this situation.
There is hope that the constraints may soon become strong enough,
thanks to large unbiased surveys of star clusters,
resolved colour-magnitude diagrams, and new analysis methods
that can account for the stochastic nature of AGB populations in clusters.

